Recursive Quantum Eigenvalue/Singular-Value Transformation: Analytic Construction of Matrix Sign Function by Newton Iteration

Quantum eigenvalue transformation (QET) and its generalization, quantum singular value transformation (QSVT), are versatile quantum algorithms that allow us to apply broad matrix functions to quantum states, which cover many of significant quantum algorithms such as Hamiltonian simulation. However, finding a parameter set which realizes preferable matrix functions in these techniques is difficult for large-scale quantum systems: there is no analytical result other than trivial cases as far as we know and we often suffer also from numerical instability. We propose recursive QET or QSVT (r-QET or r-QSVT), in which we can execute complicated matrix functions by recursively organizing block-encoding by low-degree QET or QSVT. Owing to the simplicity of recursive relations, it works only with a few parameters with exactly determining the parameters, while its iteration results in complicated matrix functions. In particular, by exploiting the recursive relation of Newton iteration, we construct the matrix sign function, which can be applied for eigenstate filtering for example, in a tractable way. We show that an analytically-obtained parameter set composed of only $8$ different values is sufficient for executing QET of the matrix sign function with an arbitrarily small error $\varepsilon$. Our protocol will serve as an alternative protocol for constructing QET or QSVT for some useful matrix functions without numerical instability.

==> Supple.tex <==
\renewcommand{\thesection}{S\arabic{section}}
\renewcommand{\theequation}{S\arabic{equation}}
\setcounter{equation}{0}
\renewcommand{\thefigure}{S\arabic{figure}}
\setcounter{figure}{0}

\onecolumngrid
\begin{center}
 {\large 
 {\bfseries Supplemental Materials for \\ ``Recursive Quantum Eigenvalue/Singular-Value Transformation; \\ Analytic Construction of Matrix Sign Function by Newton iteration'' }}
\end{center}

\begin{center}
Kaoru Mizuta$^{1,2}$ and Keisuke Fujii$^{3,4,1,5}$
\end{center}

\begin{center}
{\small 
\textit{$^1$RIKEN Center for Quantum Computing (RQC), Hirosawa 2-1, Wako, Saitama 351-0198, Japan} \\
\textit{$^2$Department of Applied Physics, The University of Tokyo, Hongo 7-3-1, Bunkyo, Tokyo 113-8656, Japan} \\
\textit{$^3$Graduate School of Engineering Science, Osaka University, \\ 1-3 Machikaneyama, Toyonaka, Osaka 560-8531, Japan.} \\
\textit{$^4$Center for Quantum Information and Quantum Biology, Osaka University, Japan.} \\
\textit{$^5$Fujitsu Quantum Computing Joint Research Division at QIQB,
\\ Osaka University, 1-2 Machikaneyama, Toyonaka 560-0043, Japan}
\\ (Dated: \today)
}
\end{center}
\vspace{20pt}

\twocolumngrid

\section{Parameter determination of QET}\label{Sec_supp:Parameter_determination}
In this section, we show how to determine the parameter set $\vec{\phi} \in \bbR^q$ in QET, for this Letter to be self-contained.
The discussion here is mainly based on Ref. \cite{Gilyen2019-qsvt}.

Suppose that we want to realize a degree-$q$ polynomial $f(x)$ satisfying (i)-(iii) in the main text by degree-$q$ QET.
This exploits a technique of quantum signal processing (QSP) \cite{Low2017-qsp}, since the achievable functions are equivalent to QET/QSVT by so-called qubitization technique \cite{Low2019-qubitization}.
We begin with determining the parameter set for QSP to realize the function $f(x)$.
QSP is a repetition of single-qubit rotation operators that embodies a polynomial function of a certain signal $x \in [-1,1]$.
A rotation-based degree-$q$ QSP operator $\mr{QSP}[x,\vec{\phi}]$ on $\bbC^2$ is defined by
\begin{eqnarray}
    \mr{QSP}[x,\vec{\phi}^\prime] &=& e^{i \phi_0^\prime Z} \prod_{i=1}^q \left[ W(x) e^{i \phi_i^\prime Z}\right], \\
    W(x) &=& \left( \begin{array}{cc}
        x & i \sqrt{1-x^2} \\
        i \sqrt{1-x^2} & x
    \end{array} \right),
\end{eqnarray}
where $\vec{\phi}^\prime \in \bbR^{q+1}$ is a tunable parameter set and $Z$ is the Pauli-$Z$ operator.
The QSP operator can be written in the form of
\begin{equation}
    \mr{QSP}[x,\vec{\phi}^\prime] = \left( \begin{array}{cc}
        f(x) & i h (x) \sqrt{1-x^2} \\
        i h^\ast (x) \sqrt{1-x^2} & f^\ast (x),
    \end{array}\right)
\end{equation}
and there exists a corresponding parameter set $\vec{\phi}^\prime \in \bbR^{q+1}$ if and only if $f(x)$ satisfies (i)-(iii) in the main text.
Then, a polynomial function $h(x)$ satisfies
\begin{enumerate}[(i$^\prime$)]
    \item $h(x)$ has a degree at most $q-1$
    \item $h(x)$ has a parity $(-1)^{q-1}$.
    \item $f(x)f^\ast(x)+(1-x^2) h(x) h^\ast (x) = 1$ for any $x$.
\end{enumerate}

To obtain a parameter set $\vec{\phi}^\prime$ for the rotation-based QSP, we should obtain the polynomial function $h(x)$.
This can be executed by finding all the roots $\{s_i \}_{i=1}^q$ of $1-f^\ast (x) f(x)$, which is a degree-$q$ polynomial in $x^2$.
From the conditions (i)-(iii) in the main text, the polynomial $1-f^\ast (x) f(x)$ is always factorized in the form of
\begin{equation}\label{Seq:Root_finding}
    1- f^\ast(x) f(x) = \alpha (1-x^2) \prod_{s_i; \mr{Im}(s_i) \geq 0} (x^2 - s_i)(x^2-s_i^\ast)
\end{equation}
with $\alpha > 0$, and thus 
\begin{equation}
    h(x) = \sqrt{\alpha} \prod_{s_i \in S; \mr{Im}(s_i) \geq 0} (x^2 - s_i),
\end{equation}
gives a proper choice satisfying (i$^\prime$)-(iii$^\prime$).

Once one obtains $h(x) = \sum_{n=0}^{q-1} h_n x^n$ for the desired polynomial $f(x) = \sum_{n=0}^q f_n x^n$, the parameter set $\vec{\phi}^\prime$ is determined in a recursive way.
We define $\phi_q^\prime$ by
\begin{equation}\label{Seq:Angle_finding}
    e^{2i \phi_q^\prime} = \frac{f_q}{h_{q-1}},
\end{equation}
and then we update the polynomials $f(x)$ and $h(x)$ by
\begin{eqnarray}
       \tilde{f}(x) &=& e^{-i \phi_q^\prime} x f(x) + e^{i \phi_q^\prime} (1-x^2) h(x) \label{Seq:degrade_fx},\\
       \tilde{h}(x) &=& e^{i \phi_q^\prime} x h(x) - e^{-i \phi_q^\prime} f(x). \label{Seq:degrade_hx}
\end{eqnarray}
The pair of $\tilde{f}(x)$ and $\tilde{h}(x)$ satisfies (i)-(iii) and (i$^\prime$)-(iii$^\prime$) for the degree $q-1$, and hence it can be realized by a degree-$(q-1)$ QSP.
The parameter $\phi_q^\prime$ is determined by Eq. (\ref{Seq:Angle_finding}) with using $\tilde{f}(x)$ and $\tilde{h}(x)$ instead of $f(x)$ and $h(x)$.
We repeat this procedure until the obtained polynomials become trivial.

Finally, we transform the angles $\vec{\phi}^\prime$ into those for QET.
With a proper choice of two-dimensional basis, QET can be identified with a reflection-based QSP operation $\bbC^2$, which is defined by
\begin{eqnarray}
    \overline{\mr{QSP}}[x,\vec{\phi}] &=& \prod_{i=1}^q \left[ e^{i \phi_i Z} R(x)\right], \quad \vec{\phi} \in \bbR^q, \\
    R(x) &=& \left( \begin{array}{cc}
        x & \sqrt{1-x^2} \\
        \sqrt{1-x^2} & -x
    \end{array}\right).
\end{eqnarray}
Namely, QET and reflection-based QSP realize the same function by $\braket{0|\mr{QET}[A,\vec{\phi}]|0}$ and $\braket{0|\overline{\mr{QSP}}[x,\vec{\phi}]|0}$ with the same angles $\vec{\phi}$.
Achievable functions by them are equivalent to those by rotation-based QSP, where we choose the angles by
\begin{equation}
    \phi_1 = \phi_0^\prime + \phi_q^\prime + (q-1)\frac{\pi}2, \quad \phi_i = \phi_{i-1}^\prime - \frac{\pi}2 \quad (2 \leq i \leq q).
\end{equation}

Numerical instability arises in the root-finding problem of the degree-$q$ polynomial, Eq. (\ref{Seq:Root_finding}), and the error is accumulated via iterative computation by Eqs. (\ref{Seq:Angle_finding})-(\ref{Seq:degrade_hx}).
In Newton-iteration-based QET, we do not suffer from them since we employ low-degree QET.
When we consider $f(x)=p_2(x)=(15x-10x^3+3x^3)/8$ to construct a matrix sign function as the main text, the factorization Eq. (\ref{Eq:Factorization_Pade_2}) analytically gives the pairwise function $h(x)$ by
\begin{equation}
    h(x) = \frac{3}{8} x^4 - \frac{1}{16} (17+3\sqrt{15}i) x^2 + \frac{1}{16}(11+3\sqrt{15}i).
\end{equation}
The iterative determination of the angles by Eqs. (\ref{Seq:Angle_finding})-(\ref{Seq:degrade_hx}) can be analytically completed, which results in Eq. (\ref{Eq:Parameter_set_Pade_2}).
We ensure the analyticity of the angles $\vec{\phi}$ also when we use the higher-order Pad\'{e} family $f(x)=p_4(x)$, where $h(x)$ can be analytically computed by the factorization,
\begin{eqnarray}
    && 1- (p_4(x))^2 = -(1-x^2)^5 \sum_{i=0}^4 a_i (x^2)^i, \\
    && a_0 = 1, \quad a_1 = -\frac{17305}{16384}, \quad a_2 = \frac{14235}{16384}, \\
    && a_3 = - \frac{6475}{16384}, \quad a_4 = \frac{1225}{16384},
\end{eqnarray}
and the quartic formula.

\section{Extension to QSVT}\label{Sec_supp:qsvt}

In this section, we briefly discuss the extension to r-QSVT, especially for the matrix sign function.
Construction similar to the main text results in QSVT with tractable parameters for polar decomposition of generic matrices.

We begin with introducing QSVT \cite{Gilyen2019-qsvt}, with restricting to odd degrees for simplicity.
For a generic finite-dimensional matrix $A \in \bbC^{d_1 \times d_2}$, its block-encoding is defined by a unitary operator $O_A$ such that
\begin{equation}
    \Pi_1 O_A \Pi_2 = A
\end{equation}
is satisfied with certain $d_1$- and $d_2$-dimensional projections $\Pi_1$ and $\Pi_2$.
With parametrized rotations designated by
\begin{equation}
    R_\phi^{\Pi_1} = e^{i\phi (2\Pi_1 - I)}, \quad R_\phi^{\Pi_2} = e^{i\phi (2\Pi_2 - I)},
\end{equation}
a degree-$q$ QSVT operator for odd $q \in \bbN$ with a parameter set $\vec{\phi} \in \bbR^q$ is defined by
\begin{equation}
    \mr{QSVT}[O_A,\vec{\phi}] = R_{\phi_1}^{\Pi_1} O_A \prod_{i=1}^{(q-1)/2} \left[ R_{\phi_{2i}}^{\Pi_2} O_A^\dagger R_{\phi_{2i+1}}^{\Pi_1} O_A \right].
\end{equation}
The matrix $A$ is always described by singular value decomposition (SVD) as $A = \sum_\sigma \sigma \ket{u_\sigma}\bra{v_\sigma}$, where $\sigma$ ($> 0$), $\ket{u_\sigma} \in \bbC^{d_1}$, and $\ket{v_\sigma} \in \bbC^{d_2}$ are respectively called a singular value, a left singular vector, and a right singular vector.
QSVT executes polynomial processing of every singular value given by
\begin{equation}
    \Pi_1 \mr{QSVT}[O_A,\vec{\phi}] \Pi_2 = \sum_\sigma f(\sigma) \ket{u_\sigma}\bra{v_\sigma},
\end{equation}
where the scalar function $f(x)$ satisfies all the conditions (i)-(iii) in the main text.
We note that this is not equal to a polynomial function $f(A)$ in general, unlike QET.

Recursive QSVT (r-QSVT) is organized completely in a similar manner to r-QET; We construct a series of unitaries $\{ O_{X_n} \}_n$ by
\begin{equation}\label{Seq:recursive_QSVT}
    O_{X_{n+1}} = \mr{QSVT}[O_{X_n},\vec{\phi}^g],
\end{equation}
which begins from a unitary $O_{X_0}$ such that $\Pi_1 O_{X_0} \Pi_2 = X_0$.
It casts a recursive relation as
\begin{eqnarray}
    X_{n+1} &=& \Pi_1 O_{X_{n+1}} \Pi_2 \nonumber \\
    &=& \sum_{\sigma_n} g(\sigma_n) \ket{u_{\sigma_n}}\bra{v_{\sigma_n}},
\end{eqnarray}
where SVD of $X_n$ is given by $X_n = \sum_{\sigma_n} \sigma_n \ket{u_{\sigma_n}} \bra{v_{\sigma_n}}$.
If we choose the function $g$ based on Newton iteration, some complicated matrix functions of $A$ will be realized.
For instance, when the parameter set $\vec{\phi}^g$ is chosen as Eq. (\ref{Eq:Pade_2}), which is given for the matrix sign function, it forms the recursive relation,
\begin{eqnarray}
    X_{n+1} &=& \sum_{\sigma_n} \frac18 (15 \sigma_n - 10 \sigma_n^3 + 3 \sigma_n^5)\ket{u_{\sigma_n}}\bra{v_{\sigma_n}} \nonumber \\
    &=& \frac18 \left\{15 - 10 (X_n X_n^\dagger) + 3 (X_n X_n^\dagger)^2 \right\} X_n, \nonumber \\
    &&
\end{eqnarray}
with $X_0 = A$.
This is nothing but the one for computing the polar decomposition $U_A \in \bbC^{d_1 \times d_2}$, which is a unitary such that $A = U_A P_A$ with a positive semidefinite matrix $P_A \in \bbC^{d_2 \times d_2}$.
Namely, we obtain $\Pi_1 O_{X_n} \Pi_2 \to U_A$ by the recursive construction Eq. (\ref{Seq:recursive_QSVT}).
Since the convergence rate is the same as the one of matrix sign functions under the assumption $^\forall \sigma \in [\Delta,1]$, the query complexity to $O_A$ to achieve an allowable error $\varepsilon$ is given by Eq. (\ref{Eq:Query_complexity_Pade_2}).

We can see the realization of polar decomposition from another aspect.
The components of the polar decomposition are respectively represented by
\begin{equation}\label{Seq:Polar_decomposition_SVD}
    U_A = \sum_\sigma \ket{u_\sigma}\bra{v_\sigma}, \quad P_A = \sum_\sigma \sigma \ket{v_\sigma}\bra{v_\sigma}.
\end{equation}
Let us consider a QSVT operator $\mr{QSVT}[O_A,\vec{\phi}]$ with organizing $\vec{\phi}$ from $\vec{\phi}^g$ as well as the matrix sign function.
When the iteration number $n$ is large enough to satisfy Eq. (\ref{Eq:Iteration_Pade_2}), QSVT processes every singular value by $f(\sigma) = \sign (\sigma) + \order{\varepsilon} = 1 + \order{\varepsilon}$.
As a result, the QSVT operator $\mr{QSVT}[O_A,\vec{\phi}]$ can accurately reproduce the polar decomposition $U_A$ given by the formula Eq. (\ref{Seq:Polar_decomposition_SVD}).
In a similar way, r-QSVT with other even-order members of Pad\'{e} family $g_{2l^\prime} (x)$ outputs the polar decomposition of generic matrices, with yielding the query complexity Eq. (\ref{Eq:Query_complexity_generic_Pade}).


\section{Quantum algorithms with \\ matrix sign function of r-QET} \label{Sec_supp:application}

In the main text, we have shown that r-QET/r-QSVT provides analytical parameter sets for matrix sign functions.
Here, we provide that the same parameter sets are available for eigenstate filtering, eigenstate preparation, and quantum linear system problems (QLSP) as a complementary result by combining the results of Ref. \cite{Lin2020-filtering_qlsp}.

\subsection{Eigenstate filtering and eigenstate preparation}
Eigenstate filtering is to filter out eigenstates having eigenenergies larger than a certain cutoff.
Assuming that a hermitian matrix $A= \sum_{a \neq 0, |a| \leq 1} a \ket{a}\bra{a}$ has a spectral gap at $a=0$, it is equivalent to apply the projection,
\begin{equation}
     P_+(A) = \frac{1+\sign (A)}{2},
\end{equation}
We use the matrix sign function generated by r-QET, such that $\braket{0|O_{X_n}|0}_b = \sign (A) + \order{\varepsilon}$.
Then, the controlled operation defined by
\begin{eqnarray}
    && O_{\Delta} (A) = \nonumber \\
    && \quad e^{i (\pi/4) Y_{b^\prime}}\left( \ket{0}\bra{0}_{b^\prime} \otimes I + \ket{1}\bra{1}_{b^\prime} \otimes O_{X_n} \right) e^{i (\pi/4) Y_{b^\prime}}. \nonumber \\
    && \label{Seq:block_encode_filtering}
\end{eqnarray}
reproduces the filtering with additional one qubit $b^\prime$ by $\braket{00|O_\Delta (A)|00}_{bb^\prime} = P_+(A) + \order{\varepsilon}$.
The query complexity in $O_A$ for the eigenstate filtering is
\begin{equation}
    \order{\Delta^{-2(1+\nu_l)} \log^{1+\nu_l} (1/\varepsilon)},
\end{equation}
when we use the matrix sign function by r-QET with the function $p_l(x)$ [See Eq. (\ref{Eq:Query_complexity_generic_Pade})].
While it is worse than the optimal cost $\order{\Delta^{-1} \log (1/\varepsilon)}$, achieved by the standard QET \cite{Lin2020-filtering_qlsp}, r-QET determines all the parameters composed of $4l+1$ different rotation angles in numerically-cheaper ways.
For instance, it requires only $9$ different rotational angles, which are analytically given by $\{\pm \phi_i\}_{i=2,3,4,5}$ in Eqs. (\ref{Eq:Parameter_set_Pade_2}) and $\pi/4$ in Eq. (\ref{Seq:block_encode_filtering}), in the simplest case $l=2$.

Eigenstate preparation is to prepare a certain isolated eigenstate of $A$ (here, we set the eigenvalue at zero).
Assuming that $A$ has no eigenvalue in $[-\Delta,\Delta]$ except for the zero eigenvalue, it is completed by applying the projection,
\begin{equation}
    P_0(A) = \ket{0}\bra{0} = P_+ \left( \frac{A+\Delta /2}{1+\Delta /2} \right) P_+ \left( - \frac{A-\Delta/2}{1+\Delta/2} \right),
\end{equation}
to a proper initial state $\ket{\psi_0}$.
In the above filtering, we use the block-encoding of $(A \pm \Delta/2)/(1+\Delta/2)$ for normalization, which requires one query to a controlled-$O_A$ operation.
We also need single-qubit unitary gates on an additional qubit, whose rotation angle is $\pm \arctan \sqrt{\Delta/2}$.
When the initial state $\ket{\psi_0}$, prepared by a unitary $U_0$, has the overlap $\gamma = |\braket{0|\psi_0}|$, r-QET with $p_l(x)$ requires
\begin{equation}
    \order{\frac{1}{\gamma} \Delta^{-2(1+\nu_l)} \log^{1+\nu_l} (1/\gamma \varepsilon)}
\end{equation}
queries to $O_A$ and $\order{\gamma^{-1}}$ queries to $U_0$.
Here, we use the amplitude amplification \cite{Martyn2021-grand-unif} which allows the quadratic speedup from the time $\order{\gamma^{-2}}$, expected by the success probability.
At the expense of the cost to some extent compared to the optimal one $\order{\gamma^{-1} \Delta^{-1}\log(1/\varepsilon)}$ \cite{Lin2020-filtering_qlsp}, r-QET works only with $4l+3$ different rotation angles.
In addition, they can be analytically obtained in the simplest cases $l=2,4$, or avoid numerical instability for larger $l$.

\subsection{Quantum linear system problem (QLSP)}
Quantum linear system problem (QLSP) is to obtain $\ket{x}=A^{-1}\ket{b}$ from a given non-singular hermitian matrix $A$ and a given vector $\ket{b}$.
Here, we define the condition number of $A$ by $\kappa = \Delta^{-1}$, and the vector $\ket{b}$ is prepared by a unitary gate $U_b$.
Recently, it has been shown that QLSP can be solved by using eigenstate filtering and eigenstate preparation as subroutines \cite{Lin2020-filtering_qlsp}.
This relies on the fact that $\ket{x}$ is obtained by an isolated eigenstate as
\begin{eqnarray}
    && \tilde{A} \left( \begin{array}{c}
        \ket{x} \\
        0
    \end{array}\right)= 0, \\
    && \tilde{A} = \left( \begin{array}{cc}
        0 & A(I-\ket{b}\bra{b}) \\
        (I-\ket{b}\bra{b}) A  & 0
    \end{array}\right).
\end{eqnarray}
The block-encoding of $\tilde{A}$ is organize by $\order{1}$ queries to $O_A$ and $U_b$.
The algorithm prepares a state having an $\order{1}$ overlap with $^\mr{t}(\ket{x},0)$ by Zeno effect reproduced by eigenstate filtering, and then make a projection onto $^\mr{t}(\ket{x},0)$ within $\order{\varepsilon}$ by eigenstate preparation in $\tilde{A}$.

In the first step, the algorithm begins with preparing the zero-energy eigenstate $^\mr{t}(\ket{b},0)$ of the trivial Hamiltonian $\tilde{A}_0 = X \otimes (I-\ket{b}\bra{b})$ 
Then, to approximately obtain the eigenstate of the target Hamiltonian $\tilde{A}$, it uses a path
\begin{equation}
    \tilde{A}(s) = f_s \tilde{A} + (1-f_s) \tilde{A}_0,
\end{equation}
with a specific scheduling function $f_s$ satisfying $f_{s=0}=0$ and $f_{s=1}=1$.
The algorithm mimics Zeno effect along this path by a series of eigenstate filtering, which is represented by
\begin{equation}
    \prod_{t=0}^{M} P_0 \left( \tilde{A}(t/M) \right)
    \left( \begin{array}{c}
        \ket{b} \\
        0
    \end{array}\right)
    = c  \left( \begin{array}{c}
        \ket{x} \\
        0
    \end{array}\right) + \dots.
\end{equation}
To achieve the overlap $c \in \order{1}$ with $^\mr{t}(\ket{x},0)$, we need $M \in \order{(\log \kappa)^2}$-times repetition and the error smaller than $\varepsilon_\mr{EF} \in \order{M^{-2}}$ of the projections $P_0$ in eigenstate filtering.
As a result, this step requires at-most
\begin{eqnarray}
    && \order{M \Delta^{-2(1+\nu_l)} \log^{1+\nu_l}(1/\varepsilon_\mr{EF})} \nonumber \\
    && \quad = \order{\kappa^{2(1+\nu_l)} (\log \kappa)^2 (\log \log \kappa)^{1+\nu_l}} %= \tilde{\mcl{O}}(\kappa^{2(1+\nu_l)})
\end{eqnarray}
queries to the unitary gates $O_A$ and $U_b$.
In order to organize the block-encoding of $\tilde{A}(s)$ for every $s=0,1/M,2/M,\hdots,1$, we also need $M+1 \in \order{(\log \kappa)^2}$ different angles, which are analytically determined by $\arctan \sqrt{f_s/(1-f_s)}$.

After the reproduction of Zeno effect by eigenstate filtering, the algorithm applies the projection $P_0(\tilde{A})$ within the allowable error $\varepsilon$.
This step yields $\order{\Delta^{-2(1+\nu_l)} \log^{1+\nu_l}(1/\varepsilon)}= \order{\kappa^{2(1+\nu_l)}\log^{1+\nu_l}(1/\varepsilon)}$ query complexity.
Due to the $\order{1}$ overlap after Zeno effect, this step outputs the accurate solution of QSLP, $\mr{t}(\ket{x}, 0)$, with $\order{1}$ success probability probability.
In total, the QLSP algorithm exploiting eigenstate filtering with r-QET is executed by
\begin{equation}
    \tilde{\mcl{O}}\left(\kappa^{2(1+\nu_l)} \log^{1+\nu_l} (1/\varepsilon)\right)
\end{equation}
queries to the unitaries $O_A$ and $U_b$.
This scaling is worse than that of the original one using the standard optimal QET for eigenstate filtering \cite{Lin2020-filtering_qlsp}, whose scaling is $\tilde{\mcl{O}}(\kappa \log (1/\varepsilon))$.
However, the algorithm based on r-QET has a strong advantage in the parameter determination also in QLSP.
While the standard one requires $\tilde{O}(\kappa \log (1/\varepsilon))$ different parameters found by numerically-unstable computation, r-QET works only with $4l+3+M+1 \in \order{(\log \kappa)^2}$ different parameters, and all of them can be found analytically or in much numerically-cheaper ways.


